Causal Discovery with Language Models as Imperfect Experts

Understanding the causal relationships that underlie a system is a fundamental prerequisite to accurate decision-making. In this work, we explore how expert knowledge can be used to improve the data-driven identification of causal graphs, beyond Markov equivalence classes. In doing so, we consider a setting where we can query an expert about the orientation of causal relationships between variables, but where the expert may provide erroneous information. We propose strategies for amending such expert knowledge based on consistency properties, e.g., acyclicity and conditional independencies in the equivalence class. We then report a case study, on real data, where a large language model is used as an imperfect expert.

==> backups/9999_backup_theoretical_results.tex <==
\section{Strategies for imperfect experts}\label{sec:methods}

% \red{TODO: move this to problem setting file}
% \subsection{Problem formulation}
% \label{sec:problem}




%\begin{align}\label{eq:problem-full-graph-soft}
%    \arg\min_{q, s} \ & \ |\Mexpert| - \log \ P(G \in \Mexpert) 
%\end{align}

\begin{itemize}
    \item include info from PC
    \item include info from LM, not calibrated and not independent identically error (iid)
    \item Tune the temperature such that GPT is calibrated. \url{https://arxiv.org/pdf/1706.04599.pdf}
    \item consistency with the MEC prior (could be replaced with other Bayesian vausal discovery)
\end{itemize}


Include knowledge of the v-structure and acyclicity using the PC algorithm then combining this with the expert knowledge.

\begin{align}
    \arg\ \max_{G' \in \Mcal_G} \  \log \ p(G')
\end{align}

where $\Mcal_G$ is the MEC of $G$ as obtained by PC.

start with max posterior

\begin{align}
    \arg\max_{G} \sum_{e \in G} \log \ p(e|o)
\end{align}

but hard threshold work best

\begin{align}
    \arg\max_{G} \sum_{e \in G} 1_{\{p(e|o)> 0.5\}}
\end{align}

where $G$ is the true DAG, $|\Mexpert|$ is the size of the equivalence class obtained by querying an expert $q$ with strategy $s$, and $\eta$ quantifies tolerance to the risk that the true graph $G$ does not belong to the resulting equivalence class.
This problem shows a clear trade-off between reducing uncertainty, by shrinking the equivalence class $\Mcal_G$, and the risk associated with making decisions based on a noisy expert.

\paragraph{Imperfect oracle}
Figure~\ref{fig:dep-graph} reports the dependency graph that we assume for the noisy expert.
For any unoriented edge indexed by $i \in [1, u]$, $E_i$ represents the (unknown) true edge orientation and $O_i$ is the orientation given by the expert.
Notice that (i) true edge orientations are in general interdependent, because of acyclicity, and that (ii) edges already oriented in the MEC are not represented as they do not affect the values of the unoriented ones.

In this model, we assume that the expert returns an orientation for an edge $i$ that depends only on its true value, i.e. $p(O_i | G) = p(O_i | E_1, \dots, E_u) = p(O_i | E_i)$.
In the following, we will be interested in estimating the probability that a subset of orientations, indexed by $I = \{i_1, \dots, i_n\}$, is correct:
$$p(E_I | O_I) = \frac{p(O_I | E_I) p(E_I)}{p(O_I)} .$$
The likelihood can be factorized as,
$$p(O_I | E_I) = \prod_{i \in I} p(O_i|E_i)$$
however, because of the interdependencies between true edge orientations, the posterior probability cannot similarly be factorized and in general $p(E_i | O_1, \dots, O_u) \neq p(E_i | O_i)$.

\input{graphmodel.tex}

\paragraph{Old version}
Assuming a perfectly calibrated expert, we can compute the probability of 

$$p(G \in \Mcal^q_G) = \prod_{e \in D} p(e|o)$$

where $e$ is the latent edge orientation, $o$ is the orientation, and $D$ is a set of orientations. The posterior can be obtained using Bayes rule:

$$p(e|o) = \frac{p(o|e)p(e)}{p(o)}$$.

$p(o|e)$ is the probability of the orientation under the expert model and $p(e)$ is a prior over the probability of an edge direction. The prior $p(e)$ can either be set to the uniform, or can be derived from the Markov Equivalence Class obtained from the PC algorithm.

\subsection{Algorithms}



\subsection{Old}

\paragraph{Relaxation: estimating interventions.} In some cases, it may be sufficient to partially recover the causal graph. 
One important example is the estimation of intervention distributions $P(X_i \mid do(X_j))$, which is ubiquitous in practical applications of causal inference (e.g., treatment effect estimation~\textbf{CITE}).
Given $G$, a number of techniques, such as \emph{do-calculus}~\textbf{CITE} and \emph{backdoor adjustment}~\textbf{CITE}, can be used to obtain an estimand for this quantity.
The latter is of particular interest, since it enables the estimation of our quantity of interest using only the causal parents of $X_j$ in $G$ (\emph{parent adjustment}).

\begin{proposition}
Let $P_{do}(X_i, X_j;~\Mexpert)$ denote the probability that there exists a graph $G' \in \Mexpert$ from which the intervention distribution can be correctly estimated. Further, let $\Ecal_{\text{pa}(X_j)}$ be the set of all edges from any $v_k$ s.t. $X_k \in pa(X_j)$ to $v_i$ in $G$. We have that $P_{do}(X_i, X_j;~\Mexpert) \geq P\left( \exists G' \in \Mexpert\text{~s.t.~}\Ecal_{\text{pa}(X_j)} \subseteq G' \right)$.
\end{proposition}

Hence, if one is solely interested in estimating intervention distributions for a pair of variables, it suffices to solve the following Problem~(\ref{eq:problem-full-graph}):
\begin{align}
    \arg\min_{q, s} \ & \ |\Mcal^{q, s}_G|\\
    \text{s.t. } & P\left( \exists G' \in \Mexpert\text{~s.t.~}\Ecal_{\text{pa}(X_j)} \subseteq G' \right) \geq 1 - \eta \nonumber,
\end{align}
where errors in orienting edges that are not part of $\Ecal_{\text{pa}(X_j)}$ are disregarded.
\ad{Should $|\Mexpert|$ still be what we minimize or should we rather minimize the uncertainty only on the edges that connect $X_j$ to its parents and children (markov blanket)}.


\subsection{Decreases the Markov Equivalence Class}

orienting one edge might decrease the MEC by 50\%.

A naive bound on the size of the Markov equivalence class $\Mcal_G$ is:
\begin{equation}
    |\Mcal_G| \leq 2^u,
\end{equation}
where $u$ corresponds to the number of unoriented edges in the corresponding CPDAG.
For any oracle-based\todo{find a better name for this} strategy, we can bound the expected size of the resulting
equivalence class using this bound and simply letting $u$ correspond to $\expect\left[ U | q, s \right]$,\todo{terrible notation right now}
which corresponds to the expected number of unoriented edges following the application of expert $q$ using strategy $s$.
For example, if the strategy leads to all unoriented edges in the CPDAG of $\Mcal_G$ to be oriented, then 
$\expect\left[ U | q, s \right] = 0$ and $\expect[|\Mcal_G^q|] \leq 2^0 = 1$, i.e., the equivalence class contains a single graph.
If this single graph were the true graph $G$, then we would say that $G$ has been identified (the ultimate goal of causal discovery).
However, the expert could have been wrong and thus, we cannot guarantee that this graph is the true graph $G$. We will need to be clever and devise strategies
to control the probability of the true graph still belonging to the resulting equivalence class. Below, we devise strategies
that present a tradeoff between the size of the resulting equivalence class and the probability that $G$ is included in it.

\subsection{Strategy: naive application of the expert}
\vale{The problem with the following results is that the probability of the true graph being in the reduced MEC decreases with the number of oriented edges $K$}
Always believing the expert and breaking ties arbitrarily

$$p(G \in \Mcal^q_G) = \prod_k (1-\epsilon_k)$$

where $\epsilon_k$ is the probability of the expert being wrong about the direction of the edge between $v_i$ and $v_j$.

\subsection{More sophisticated approach}

Instead of naively agreeing with the expert on every decision, we can make sophisticated decisions. 

$$p(G \in \Mcal^q_G) = \prod_{d \in D} (1-\epsilon_d)$$

where $d$ refers to decision D and $\epsilon_d$ refers to the probability of decision $d$ being wrong.

\subsection{Strategy: orient on chain-consensus only}

In section~\ref{sec:problem}

\red{AD: added this without looking at the previous section for now. I derived the proba of error and orientation for this strategy. We can get proba of error and bounds on exp size of mec. I will add later today.}


==> backups/background.tex <==
% \paragraph{Expert knowledge:} The goal of incorporating expert knowledge into causal discovery is to eliminate all graphs that are deemed to be implausible by an expert. Previous work has considered expert knowledge under the form of: (i) forbidden edges~\citep{meek1995}, i.e., causal relationships that are known not to exist, (ii) (partial) orderings of the variables~\citep{scheines1998tetrad,andrews2020} and ancestral constraints~\citep{decampos2007bayesian,li2018bayesian,chen2016learning}, i.e., knowledge that one variable is measured before another, and (iii) constraints on interactions between types of variables~\citep{brouillard2022typing} (e.g., symptoms do not cause a disease). See \citet{constantinou2023impact} for an overview.
% While some previous work incorporates such information as a soft constraint (e.g., \citet{mukherjee2008network}), most enforce it through hard constraints and discard incompatible graphs altogether.
% This is problematic since, realistically, expert knowledge is unlikely to be always correct, which can lead to the problematic case where $\trueg \not\in \Mexpert{~}$.
% In this work, we attempt to reduce the size of the MEC as much as possible, i.e., $\lvert\Mexpert{~}\lvert \ll \lvert\Mcal_G\lvert$, with probability $p(\trueg \in \Mexpert{~})$ high, in the presence of imperfect expert knowledge.
% We note that our work is akin to \citet{oates2017}, but that a key difference is that we do not assume that the expert is \emph{directionally informed}, i.e., that it never returns the opposite orientation for an edge in $\trueg$.
% Further, their approach is \emph{expert-first}, i.e., the expert posits an initial causal graph and the data is used to extend it, while our approach is \emph{data-first}, i.e., the expert is used to resolve uncertainty in the solution of a causal discovery algorithm.


\textbf{Large language models:~~} 
% TODO (don't forget LM priors)
% \red{The previous section feeds into this one by saying that human experts can be costly or unavailable. LLMs contain a lot of world knowledge so it would be nice to use them to augment causal discovery. However, they are most likely to be wrong in many cases. So we need approaches that can handle this noise.}
Although extremely valuable, eliciting human experts can be costly, time-consuming, and/or infeasible. Large Language Models (LLMs) offer promise in mitigating these challenges and informing causal discovery by leveraging their rich knowledge base. 
In practice, LLMs can be prompted using the \textit{metadata} associated with the variables in a causal graph to extract insights into causal relationships~\citep{long2023, willig2022can, lmpriors,  kiciman2023causal, hobbhahn2022investigating, tu2023causaldiscovery}. Reasoning with said metadata is akin to experts using the variable name, problem context, and their knowledge expertise to construct the causal structure. Like human experts, LLMs are also imperfect, possibly misattributing the direction or presence of an edge and making basic causal errors. Nevertheless, approaches such as LMPriors \cite{lmpriors} have been shown to achieve superior results on T\u{u}ebigen pairwise causal discovery problems~\citep{JMLR:v17:14-518}. 
% Such, LMPriors \cite{lmpriors} presents a framework for incorporating metadata from the rich knowledge base of LLMs as a way to construct \textit{task-specific priors} for use in any learning setting with natural language descriptions of the variables of interest. In a special case of binary hypothesis testing, LMPriors can be used to elicit the posterior probability of potential relationships between two variables x and y:  \begin{math}X \rightarrow Y (H_{0})\end{math} or \begin{math}Y \rightarrow X (H_{1})\end{math}. Thus in this context, returning (log) posterior probability for the most likely causal relationship between x and y. LMPriors alone outperformed the RECI algorithm on identifying the correct causal direction between T\u{u}ebigen pairs \cite{lmpriors}, achieving accuracy's of 84.5\% and 58.7\%, respectively. 
Unlike existing LLM-based methods, this work aims to amend potential expert misorientations by considering longer causal chains (i.e., accounting more than two variables) and incorporating consistency rules induced by the true MEC.
% Our approach can be used to handle the noise that accompanies an LLM. 


%Evaluating the utility of LLMs in uncovering causal relationships and causal reasoning has been the focus of much recent work \cite{kıcıman2023causal, willig2022can, cox2023, zhang2023understanding, long2023}. In the context of simple medical DAGs comprised of 3-4 nodes, \citet{long2023} illustrated the value of prompt tuning in whether the LLM inferred the presence or absence of an edge between two pairwise variables. While \citet{kıcıman2023causal} showed the importance of probing reasoning of LLMs -when determining the causal direction (\begin{math} A \longrightarrow B \end{math} or \begin{math}B \longrightarrow A \end{math}) between T\u{u}ebigen pairs with varying prompts (weighted accuracy 0.87-0.97). 

==> backups/problem_setting.tex <==
\section{Problem Setting}\label{sec:problem}

We now formalize our problem of interest.
Let $\trueg = \left<\Vcal_\trueg, \Ecal_\trueg \right>$ be a causal graph, as defined in \cref{sec:background}, and let $\Mcal_\trueg$ be its Markov equivalence class. We assume the availability of \emph{metadata} $\{\mu_1, \ldots, \mu_d\}$, where each $\mu_i$ provides some information about $X_i$, e.g., a name, a brief description, etc.

% In contrast with the standard causal discovery setting, we consider that each variable in $G$ is accompanied by metadata defined as follows:

% We aim to reduce uncertainty on $G$ by querying an expert to orient edges whose orientation varies in $\Mcal_G$, i.e., $\exists G_k, G_l \in \Mcal_G$ s.t. $(v_i, v_j) \in \Ecal_{G_k}$ and $(v_j, v_i) \in \Ecal_{G_l}$, resulting in a new equivalence class $\Mexpert$, s.t. $\lvert \Mexpert \lvert < \lvert\Mcal_G\lvert$, where either $G_k$ or $G_l$ is excluded.
% However, we must not exclude $G$.
% Consider the following definitions:

% Our goal is to use an expert $E$ to orient edges whose orientation varies among members of $\Mcal_G$, i.e., to find $\Mexpert$, s.t., $G \in \Mexpert$ and $\lvert\Mexpert\lvert < \Mcal_G$. The main challenge comes from the fact that the expert is \emph{imperfect}. If the expert incorrectly orients an edge, the resulting equivalence class will not contain $G$, i.e., $\Mexpert \not\subseteq \Mcal_G$.

% The rest of the presentation assumes that $\Mcal_G$ is known.
% However, in practice, our methodology could be applied to the output of any causal discovery algorithm.

% \begin{definition}
% \textbf{(Variable metadata)} We assume that each variable $X_i \in \Vcal_G$ is accompanied by metadata $\mu_i$ of arbitrary nature (e.g., a name, a brief description, etc.).
% \end{definition}

We then assume access to an expert, who consumes such metadata and makes decisions, defined as follows:
\begin{definition}
\textbf{(Expert)} An expert is a function that, when queried with the metadata for a pair of variables $(\mu_i, \mu_j)$, returns a hypothetical orientation for the $X_i - X_j$ edge:
\begin{equation}
    E\left(\mu_i, \mu_j \right) = \left\{
    \begin{array}{ll}
    		\rightarrow  & \mbox{if it believes that } (v_i, v_j) \in \Ecal_\trueg \\
    		\leftarrow & \mbox{if it believes that } (v_j, v_i) \in \Ecal_\trueg\\
    \end{array}\right.
\end{equation}
\end{definition}

Of note, $E\left(\mu_i, \mu_j \right)$ can be incorrect (imperfect expert) and thus, our problem of interest consists in
elaborating strategies to maximally make use of such imperfect knowledge.
% Possible instantiations include a human, but could also consist of a question-answering system coupled with a knowledge base and even a large-language model.

% \textbf{Variable metadata:~} In contrast with the standard causal discovery setting, we assume that each variable $X_i$ is accompanied by metadata $\mu_i$ of arbitrary nature (e.g., a name, a brief description, parameters of a measurement device, etc.).

% \textbf{Imperfect expert:~} We assume access to a domain expert which, when queried using the metadata that describes a pair of variables $(m_i, m_j)$, returns its expert opinion on the orientation of an edge between these variables. Such an expert can be human, but could also consist of a question-answering system coupled with a knowledge base and even a large-language model. Formally, we denote a query to the expert by a function $q$, such that 
% \begin{equation}
%     E\left(\mu_i, \mu_j \;\; ; \;\; \Ccal \right) = \left\{
%     \begin{array}{ll}
%     		\rightarrow  & \mbox{if it believes that } (v_i, v_i) \in \Ecal_G \\
%     		\leftarrow & \mbox{if it believes that } (v_j, v_i) \in \Ecal_G\\
%     \end{array}\right.
% \end{equation}
% where $\Ccal$ denotes an arbitrary set of context-specifying covariates (e.g., parameters that control how queries are presented to the expert).
% Of note, we do not assume that the expert has perfect knowledge and thus, such queries do not always return the correct orientation for causal relationships.
More precisely, we assume that $\mathcal{M}_\trueg$ is known\footnote{e.g., it could be obtained via some causal discovery algorithm.} and focus on using the expert to orient edges between pairs of variables $\unor \subseteq \Vcal_\trueg \times \Vcal_\trueg$ for which the causal orientation is ambiguous in $\Mcal_\trueg$, i.e., $\forall (X_i, X_j)$ s.t. $\exists G_k, G_l \in \Mcal_\trueg$ s.t. $(v_i, v_j) \in \Ecal_{G_k}$ and $(v_j, v_i) \in \Ecal_{G_l}$. We aim to elaborate a strategy $S$ to incorporate the expert's knowledge and obtain a new equivalence class $\MexpertS{~}$, such that uncertainty is reduced to the minimum, i.e., $\lvert \MexpertS{~} \lvert \ll \lvert\Mcal_\trueg\lvert$, but $\trueg$ still belongs to $\MexpertS{~}$ with high probability, that is:
\begin{align}\label{eq:problem-full-graph}
    \min \ & \ \left\lvert\MexpertS{~}\right\lvert\\
    \text{such that} & \ p\left(\trueg \in \MexpertS{~}\right) \geq 1 - \eta \nonumber,
\end{align}
% \begin{align}\label{eq:problem-full-graph}
%     \min_S \ & \ \left\lvert\MexpertS{~}\right\lvert\\
%     \text{such that} & \ \mathbb{P}\left[G \in \MexpertS{~}\right] \geq 1 - \eta \nonumber,
% \end{align}
where $\eta \in [0, 1]$ quantifies tolerance to the risk that the true graph $\trueg$ does not belong to the resulting equivalence class.
This problem can be read as a trade-off between reducing uncertainty, by shrinking the set of plausible DAGs, and the risk associated with making decisions based on an imperfect expert model.
In the next section, we formalize how we estimate the risk of incorrectly orienting a set of edges and propose strategies to address Problem\eqref{eq:problem-full-graph}.

% We aim to reduce uncertainty on $G$ by querying an expert $E$ to orient edges whose orientation is uncertain in $\Mcal_G$, i.e., $\exists G_k, G_l \in \Mcal_G$ s.t. $(v_i, v_j) \in \Ecal_{G_k}$ and $(v_j, v_i) \in \Ecal_{G_l}$.
% We then aim to incorporate the expert's knowledge using a strategy $S$, to rule out some graphs in $\Mcal_G$ and obtain a new equivalence class, $\MexpertS{G}$, such that uncertainty is reduced to the minimum, i.e., $\lvert \MexpertS{G} \lvert \ll \lvert\Mcal_G\lvert$, but $G$ still belongs to $\MexpertS{G}$.
% This results in the following optimization problem:
% We are interested in reducing uncertainty on the causal graph to the minimum, while controlling the probability of $G$ not belonging to the resulting equivalence class. As such, we seek to elaborate a strategy $S$ to incorporate $E$, while solving the following constrained optimization problem: %, such that we want to minimize the size of the MEC while the probability of the true graph being in the MEC is at least $1-\eta$.

% \red{This section is missing something about assumptions we make on the expert (independent errors and epsilon probability). This could probably be done through a definition right under the expert one.}

% \begin{algorithm}
% \caption{Our causal discovery algorithm which uses data from LLMs as priors to update}\label{alg:cap}
% \begin{algorithmic}[1]
% \Require Undirected graph with fully connected edges
% \State Apply PC Algorithm \par
%     \State Output: Partially oriented DAG (CP-DAG)
%     \For{Each CP-DAG} 
%         \State Test pairwise adjacent nodes (variables) by asking GPT-3:
%         \State "Does X cause Y?"
%         \State "Does Y cause X"?

% \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}




==> backups/theoretical_results.tex <==
\section{Strategies for imperfect experts}\label{sec:methods}

% \red{Valentina could you please fill this section? I think a good plan would be to start with the postulated noise model and then present the two greedy algorithms + global scoring (if we want to include it).}

% \begin{itemize}
%     \item include info from PC
%     \item include info from LM, not calibrated and not independent identically error (iid)
%     \item Tune the temperature such that GPT is calibrated. \url{https://arxiv.org/pdf/1706.04599.pdf}
%     \item consistency with the MEC prior (could be replaced with other Bayesian vausal discovery)
% \end{itemize}

Instead of blindly accepting expert orientations, we leverage the consistency information provided by the true MEC to estimate which decisions are most likely incorrect. 
Indeed, among all possible combinations of edge orientations, only a few are consistent with the true MEC (i.e., there exists a DAG that contains such orientations) because many of them would create cycles or new v-structures. 
The different strategies that we now propose for solving Problem~\eqref{eq:problem-full-graph} leverage such consistency imperatives in order to reduce the risk of errors.
They also assume the following noise model for the orientations provided by the expert.

\paragraph{Epsilon expert}
Figure~\ref{fig:dep-graph} shows the dependency graph that we assume for the imperfect expert, that we dub "epsilon-expert".
For any unoriented edge indexed by $i \in [1, |\unor|]$, $O_i$ represents the (unknown) true edge orientation and $E_i = E(\unor_i)$ the orientation given by the expert.
Notice that (i) true edge orientations are in general interdependent, because of the mentioned consistency information, and that (ii) edges already oriented in the MEC are not represented as they do not affect the values of the unoriented ones.
In this model, we assume that the expert returns an orientation for an edge $i$ that depends only on its true value, i.e. $p(E_i | \trueg) = p(E_i | O_1, \dots, O_{|\unor|}) = p(E_i | O_i)$ and with constant probability of error $p(E_i \neq O_i) = \varepsilon$.

In the following, we will be interested in estimating the posterior probability that a subset of oriented edges, indexed by $I  \subseteq \unor$, is correct:
$$p(O_I | E_{\unor}) = \frac{p(E_{\unor} | O_I) p(O_I)}{p(E_{\unor})}, $$
given the chosen prior $p(O_I)$.
Note that this corresponds to $p\left(\trueg \in \MexpertS{~}\right)$ since any mistake in orienting an edge in $I$ would result in excluding $G$ from the resulting MEC.
% Note that this posterior corresponds to the probability $p\left(\trueg \in \MexpertS{~}\right) = p\left(O_{I}\in \MexpertS{~}\right)p\left(O_{\unor \setminus I}\in \MexpertS{~}\right) = p\left(O_{I}\in \MexpertS{~}\right)$.
% $\unor \setminus I = \Ucal(\MexpertS{~})$
The assumption that the expert makes independent errors allows us to factorize its likelihood as,
$$p(E_I | O_I) = \prod_{i \in I} p(E_i|O_i).$$
However, because of the interdependencies between true edge orientations, the posterior probability cannot similarly be factorized and in general $p(O_i | E_{\unor}) \neq p(O_i | E_i)$.

\input{graphmodel.tex}

\paragraph{Greedy approach}
We propose a greedy strategy for optimizing Problem~\eqref{eq:problem-full-graph} that, while the risk of making an error remains below the chosen tolerance level $\eta$, iteratively orients a subset of edges.
Let $\Mcal^{(t)}$ denote the MEC at the t-th iteration of the algorithm and let $\Mcal^{(t)}_i$ denote the MEC resulting from orienting the edge between the $i$-th element of $\unor$ at step $t$.
% At a given iteration $t$, the subsets of orientations to chose from are given by an orientation of an edge still undecided so far ($E_i \in \Mexpertg{(t)}$) and all orientations subsequently 
At a given iteration $t$, we choose to orient an edge $(u_i, u_j) \in \Ucal(\Mcal^{(t)})$ according to $E(u_i, u_j)$ and apply Meek rules~\citep{meek1995} to propagate other orientations resulting from this one to obtain $\Mcal^{(t)}_i$.
% that either (\textit{MEC}) allows us to reduce the MEC size the most or (\textit{confidence}) is the most likely to be correct.
We consider two strategies to select the best $i$: 
\begin{enumerate}
    \item MEC: $\arg\min_i | \Mcal^{(t)}_i | $
    \item Risk: $\arg\min_i \left[ 1 - P\left(O_{\unor \setminus \Ucal\left(\Mcal^{(t)}_i\right)} \mid E_{\unor}\right) \right]$
\end{enumerate}

% implied by it (the set of orientations that are common to all remaining DAGs in the new MEC $I_{t} = \unor \setminus \mathcal{U}(\Mexpertg{t, \overset{\rightarrow}{i}})$).
% The risk of a subset of orientation is then $p(O_I| E_I)$.

\paragraph{Choice of prior} 
MEC prior (marginalize over all combinations of non-oriented edges): 
$$ p(O_I) = \sum_{\{o_j\}_{j \notin I} \in \Mcal_\trueg} p(O_I, O_1 = o_1, O_2 = o_2, \dots, O_{\unor \setminus I})$$
Independent prior ($p(O_{I=\{i\}})$ from above): $$ p(O_I) = \prod_{i \in I} p(O_i)$$
% Include knowledge of the v-structure and acyclicity using the PC algorithm then combining this with the expert knowledge.

%\begin{align}
%    \arg\ \max_{G' \in \Mcal_G} \  \log \ p(G')
%\end{align}%

%where $\Mcal_G$ is the MEC of $G$ as obtained by PC.%

%start with max posterior%

%\begin{align}
%    \arg\max_{G} \sum_{e \in G} \log \ p(e|o)
%\end{align}%

%but hard threshold work best%

%\begin{align}
%    \arg\max_{G} \sum_{e \in G} 1_{\{p(e|o)> 0.5\}}
%\end{align}

%%\paragraph{Old version}
%Assuming a perfectly calibrated expert, we can compute the probability of 
%
%$$p(G \in \Mcal^q_G) = \prod_{e \in D} p(e|o)$$
%
%where $e$ is the latent edge orientation, $o$ is the orientation, and $D$ is a set of orientations. The posterior can be obtained using Bayes rule:
%
%$$p(e|o) = \frac{p(o|e)p(e)}{p(o)}$$.
%
%$p(o|e)$ is the probability of the orientation under the expert model and $p(e)$ is a prior over the probability of an edge direction. The prior $p(e)$ can either be set to the uniform, or can be derived from the Markov Equivalence Class obtained from the PC algorithm.
%


==> old.tex <==
\begin{table}[ht]
    \centering
\begin{tabular}{l|lr}
\toprule
\textbf{Edge} & \textbf{Querying GPT} &  \textbf{Greedy Search}\\
\midrule
Birth asphyxia $\rightarrow$ disease & X &      \textbf{\textcolor{Green}{$\surd$} } \\

          \hline
Disease $\rightarrow$ sick & X &   X    \\          
\hline
Disease $\rightarrow$ duct flow & X & \textcolor{Green}{$\surd$}      \\

            \hline
Disease $\rightarrow$ cardiac mixing & X & \textcolor{Green}{$\surd$}     \\

            \hline
Disease $\rightarrow$ lung parenchyma & X &   X \\

            \hline
Disease $\rightarrow$ lung flow & X &   \textcolor{Green}{$\surd$} \\

            \hline
Disease $\rightarrow$ left ventricular\\hypertrophy & X &  \textcolor{Green}{$\surd$} \\

            \hline
Disease $\rightarrow$ age & X &     X \\

            \hline
Sick $\rightarrow$ age & X &     \textbf{} \\

            \hline
Sick $\rightarrow$ grunting & X &     \textbf{} \\

            \hline      
Duct flow $\rightarrow$ Hypoxia distribution & X &     \textbf{} \\

            \hline
Cardiac mixing $\rightarrow$ oxygen hypoxia & X &     \textbf{} \\

            \hline
Cardiac mixing $\rightarrow$ hypoxia distribution & X &     \textbf{} \\

            \hline
Lung parenchyma $\rightarrow$ grunting & \textcolor{Green}{$\surd$}  &     \textbf{} \\

            \hline
Lung parenchyma $\rightarrow$ oxygen hypoxia & X &     \textbf{} \\

            \hline
Lung parenchyma $\rightarrow$ CO2 & \textcolor{Green}{$\surd$}  &     \textbf{} \\

            \hline
Lung parenchyma $\rightarrow$ chest x-ray & X &     \textbf{} \\

            \hline
Lung flow $\rightarrow$ chest x-ray & X &     \textbf{} \\

            \hline
left ventricular\\hypertrophy$\rightarrow$ LVH report & X &  X \\

            \hline
Grunting $\rightarrow$ grunting report & X &     \textbf{} \\

            \hline
Hypoxia distribution$\rightarrow$ oxygen levels in \\lower body & X &     \textbf{} \\

            \hline
Oxygen hypoxia $\rightarrow$ oxygen levels in \\lower body & \textcolor{Green}{$\surd$} &     \textbf{} \\

            \hline
Oxygen hypoxia $\rightarrow$ oxygen levels in \\lower quadriceps & X &     \textbf{} \\

            \hline
CO2 $\rightarrow$ CO2 report & X &    \textcolor{Green}{$\surd$} \\

            \hline
Chest x-ray 	$\rightarrow$ x-ray report & X &     \textbf{} \\

            \hline
\bottomrule
\end{tabular}
    \caption{Comparison of which approach gets which edges correct or not. Querying GPT3 via X causes Y. Check = correctly oriented edge; X = incorrectly oriented edge; empty cell = no decision made}
    \label{tab:baselines}
\end{table}


